ASTERISM: Do Multimodal LLMs Actually Look at All the Images?

Multi-image benchmarks aim to test whether a multimodal large language model (MLLM) combines evidence across images, but many of their items can be answered from a single image. Across about 33k items from 19 public benchmarks, our audit and a two-stage single-image filter find that one image or the question alone settles 24.2% of them. On these items, MLLMs recover from one image a median 78% of the accuracy that all images add over the text alone, so these items reward answering from one image, which we call the single-image shortcut. MLLMs take this shortcut even on items where one image is not enough. On such items, most of their wrong answers repeat an answer they give from one image, at a rate well above chance. We build ASTERISM, to our knowledge the largest audited multi-image benchmark, from these 19 benchmarks by keeping their items that need more than one image. Its 18.7k items, 2.0k of them corrected or rewritten, share one format, one scorer and seven task categories. We also release ASTERISM-Train with 49k training items and ASTERISM-Lite, a hard subset whose items we manually verify one by one. On ASTERISM-Lite, the strongest proprietary MLLM scores 68%. Reinforcement learning with verifiable rewards (RLVR), now common in MLLM post-training, rewards the shortcut as well, because a correct answer read off one image earns as much reward as one that combines images. In line with this, existing RLVR objectives add little to the ASTERISM score. To stop rewarding the shortcut in training as ASTERISM does in evaluation, we propose cross-image credit assignment (CICA), an extension of RLVR that moves the credit toward the tokens that need more than one image. On three open-source MLLMs, CICA raises the ASTERISM score by 2.6 to 6.0 points, more than twice the gain of each general and vision-specific RL objective trained on the same data.

==> preamble.tex <==
\usepackage{cuted}


\usepackage{caption}
\makeatletter\newcommand{\inlinetables}{\renewenvironment{table}[1][]{\def\@captype{table}}{}}\makeatother


\usepackage{algorithm}
\usepackage{placeins}
\usepackage{adjustbox}
\usepackage{tabularx}
\usepackage{algpseudocode}

\setcounter{dbltopnumber}{2}\setcounter{topnumber}{3}\setcounter{totalnumber}{4}
\renewcommand{\dbltopfraction}{0.9}\renewcommand{\topfraction}{0.9}\renewcommand{\textfraction}{0.07}\renewcommand{\floatpagefraction}{0.8}\renewcommand{\dblfloatpagefraction}{0.8}
\setlength{\textfloatsep}{10pt plus 2pt minus 2pt}\setlength{\dbltextfloatsep}{10pt plus 2pt minus 2pt}\setlength{\floatsep}{8pt plus 2pt minus 2pt}\setlength{\dblfloatsep}{8pt plus 2pt minus 2pt}
\usepackage{microtype}
\setlength{\textfloatsep}{7pt plus 2pt minus 2pt}\setlength{\dbltextfloatsep}{7pt plus 2pt minus 2pt}\setlength{\intextsep}{8pt plus 2pt minus 2pt}
\captionsetup{skip=4pt}
\makeatletter
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}{0.3em \@plus 0.1em \@minus 0.1em}{-0.6em}{\normalfont\normalsize\bfseries}}
\def\cvprsection{\@startsection {section}{1}{\z@}{-7pt plus -2pt minus -2pt}{4pt} {\large\bf}}
\def\cvprsubsection{\@startsection {subsection}{2}{\z@}{-5pt plus -2pt minus -1pt}{3pt} {\elvbf}}
\setlength{\parskip}{0pt}
\makeatother

